The Web Is Your Oyster - Knowledge-Intensive NLP against a Very Large Web Corpus

In order to address increasing demands of real-world applications, the research for knowledge-intensive NLP (KI-NLP) should advance by capturing the challenges of a truly open-domain environment: web-scale knowledge, lack of structure, inconsistent quality and noise. To this end, we propose a new setup for evaluating existing knowledge intensive tasks in which we generalize the background corpus to a universal web snapshot. We investigate a slate of NLP tasks which rely on knowledge - either factual or common sense, and ask systems to use a subset of CCNet - the Sphere corpus - as a knowledge source. In contrast to Wikipedia, otherwise a common background corpus in KI-NLP, Sphere is orders of magnitude larger and better reflects the full diversity of knowledge on the web. Despite potential gaps in coverage, challenges of scale, lack of structure and lower quality, we find that retrieval from Sphere enables a state of the art system to match and even outperform Wikipedia-based models on several tasks. We also observe that while a dense index can outperform a sparse BM25 baseline on Wikipedia, on Sphere this is not yet possible. To facilitate further research and minimise the community's reliance on proprietary, black-box search engines, we share our indices, evaluation metrics and infrastructure.

==> images/downstream_change/Makefile <==
all:
	gnuplot script_aic_web_multi.gnuplot  && epstopdf chart.eps && pdfcrop chart.pdf && rm chart.eps && rm chart.pdf && mv chart-crop.pdf aic_web_multi.pdf && \
	gnuplot script_aeic_web_multi.gnuplot  && epstopdf chart.eps && pdfcrop chart.pdf && rm chart.eps && rm chart.pdf && mv chart-crop.pdf aeic_web_multi.pdf && \
	gnuplot script_aic_web_bm25.gnuplot  && epstopdf chart.eps && pdfcrop chart.pdf && rm chart.eps && rm chart.pdf && mv chart-crop.pdf aic_web_bm25.pdf
	gnuplot script_aeic_web_bm25.gnuplot  && epstopdf chart.eps && pdfcrop chart.pdf && rm chart.eps && rm chart.pdf && mv chart-crop.pdf aeic_web_bm25.pdf

==> tables/index_dev.tex <==
\begin{table*}[t!]
\centering
\resizebox{\linewidth}{!}{    
    \fontsize{8.4}{10.1}\selectfont \setlength{\tabcolsep}{0.5em}
\begin{tabular}{c|ccc|ccc|ccc|ccc|ccc}
 
\toprule
 & \multicolumn{3}{c}{\textbf{T-REx}} & \multicolumn{3}{c}{\textbf{zsRE}}  & \multicolumn{3}{c}{\textbf{NQ}} & \multicolumn{3}{c}{\textbf{HoPo}} & \multicolumn{3}{c}{\textbf{TQA}} \\
\midrule
k & 1 & 20 & 100 & 1 & 20 & 100 & 1 & 20 & 100 & 1 & 20 & 100 & 1 & 20 & 100 \\
\midrule

HNSW-SQ8 & 57.5 &  78.12 & 83.84 & 28.44 & 54.73 & 66.14 & 53.61 & 83.12 & 89.25 & 30.30 & 59.77 & 70.48 & 78.99 & 96.08 & 98.11 \\
flat &  61.18 &  82.22 & 88.08 & 33.75 & 62.67 & 73.87 & 55.62 & 86.18 & 92.49  & 32.43 & 63.16 & 74.14 & 80.48 & 97.26 & 98.99 \\


\bottomrule
\end{tabular}
}
\caption{Answer-in-context@k for two types of CC-NET indices}
\label{tab:index_dev}
\end{table*}


==> tables/raw_examples_trivia_fever.tex <==
TRIVIA_QA

For how many years was Richard III king of England?
web asnwer: two
wiki asnwer: 1483

web provenance:
 King Richard III remains one of the most infamous and recognisable monarchs in English or British history, despite only sitting on the throne for two years and fifty-eight days. Fact and Fictions King Richard III remains one of the most infamous and recognizable monarchs in English or British history, despite only sitting on the throne for two years and fifty-eight days. His hold on the popular imagination is largely due to the fictional portrayal of him by William Shakespeare which, combined with the workings of five centuries of rumor and gossip, has created two opposing versions of Richard. In fiction
https://www.casemateipm.com/subject-categories/biography-autobiography/royalty/richard-iii.html

wiki provenance:
 was then carried back to Leicester tied to a horse, and early sources strongly suggest that it was displayed in the collegiate Church of the Annunciation of Our Lady of the Newarke, prior to being buried at Greyfriars Church in Leicester. In 1495, Henry VII paid for a marble and alabaster monument. According to a discredited tradition, during the Dissolution of the Monasteries, his body was thrown into the River Soar, although other evidence suggests that a memorial stone was visible in 1612, in a garden built on the site of
Richard III of England




In religion, there are how many Stations of the Cross?
web asnwer: fourteen
wiki asnwer: eight

web provenance:
 There are 14 Stations of the Cross in every Catholic Church. At each station there is a painting or statue depicting Jesus Christ as He is led to His crucifixion and death. During the time of the crusades (1095-1270), pilgrims to the Holy Land followed the path of Jesus to Calvary. After the Moslems captured the Holy Land, the Way of the Cross... held outdoors... became a substitute pilgrimage throughout Europe. In the l8th century Stations were allowed inside churches. Eventually, fourteen Stations became a familiar feature in Catholic churches. The Way of the Cross makes us more aware of
https://www.comeaside.com/stations-of-the-cross.html

wiki provenance:
 time 8. Jesus meets the women of Jerusalem 9. Jesus falls for the third time 10. Jesus is stripped of His clothes 11. Jesus is nailed to the cross 12. Jesus dies on the cross 13. Jesus is taken down from the cross 14. Jesus is placed in the tomb Although not traditionally part of the Stations, the Resurrection of Jesus is, in very rare instances, included as a fifteenth station. Stations Scriptural form. Out of the fourteen traditional
Stations of the Cross




What is the title of the film considered to be the debut of cartoon character Mickey Mouse?
web asnwer: steamboat willie
wiki asnwer: plane crazy

web provenance:
 in the world. Mickey first was seen in a single test screening (Plane Crazy). Mickey officially debuted in the short film Steamboat Willie (1928), one of the first sound cartoons. He went on to appear in over 130 films, including The Band Concert (1935), Brave Little Tailor (1938), and Fantasia (1940). Mickey appeared primarily in short films, but also occasionally in feature-length films. Ten of Mickey's cartoons were nominated for the Academy Award for Best Animated Short Film, one of which, Lend a Paw, won the award in 1942. In 1978, Mickey became the first cartoon character to have a
http://www.worldlibrary.org/articles/eng/Mickey_Mouse

wiki provenance:
 The Pointer" (1939) - "The Nifty Nineties" (1941) - "Lend a Paw" (1941) - "Symphony Hour" (1942) - "Squatter's Rights" (1946) - "Mickey and the Seal" (1948) - "The Simple Things" (1953) - "Mickey's Christmas Carol" (1983) - "Runaway Brain" (1995) - "Get a Horse!" (2013) Filmography Full-
Mickey Mouse



FEVER


Tenacious D started in 1997.
web asnwer: REFUTES
wiki asnwer: SUPPORTS

web provenance:
 Tenacious D is an American rock band that was formed in Los Angeles, California in 1994. Composed of lead vocalist and guitarist Jack Black and lead guitarist and vocalist Kyle Gass, the band has released two albums – Tenacious D (2001) and The Pick of Destiny (2006). The band's studio releases, and more recently its live performances, feature a full band lineup, including such musicians as guitarist John Konesky, bassist John Spiker and Bad Religion drummer Brooks Wackerman. Tenacious D formed in 1994 when the members performed as an acoustic duo. The band first gained popularity in 1999 when they
http://events.stuff.co.nz/artist/tenacious-d

wiki provenance:
 Tenacious D (album) Tenacious D is the first studio album by American comedy rock band Tenacious D, released on September 25, 2001 by Epic Records. The album's polished production was a departure from the band's acoustic origins, due in part to the production of the Dust Brothers. "Tribute" was the first single released from the album, followed by "Wonderboy". Both singles had music videos filmed for them, with the Liam Lynch–directed Tribute video achieving cult status. While "Tenacious
Tenacious D (album)



Harold Macmillan died on December 29, 1886.
web asnwer: REFUTES
wiki asnwer: SUPPORTS

web provenance:
 Harold Macmillan, the grandson of Daniel Macmillan, the publisher, was born in 1894. Educated at Eton and Balliol College, Oxford. On the outbreak of the First World War, Macmillan left university and joined the Grenadier Guards. He served on the Western Front where he was wounded three times. After the Armistice, Macmillan joined the family publishing company but in the 1924 General Election he became the Conservative MP for Stockton-on-Tees. Defeated in the 1929 General Election he returned in to the House of Commons in 1931. Macmillan was a strong believer in social reform and his left-wing views were unpopular
https://www.panmacmillan.com/authors/harold-macmillan/a1ce0b04-b14d-4882-7468-08d5dd189b1f

wiki provenance:
 , he died at the age of 92. Macmillan was the last British prime minister born during the Victorian era, the last to have served in the First World War and the last to receive a hereditary peerage. At the time of his death, he was the longest-lived prime minister in British history, a record surpassed by James Callaghan on 14 February 2005. Early life. Early life Family. Macmillan was born at 52 Cadogan Place in Chelsea, London, to Maurice Crawford Macmillan (1853–1936)
Harold Macmillan





Michelin Guides have been published for more than a decade.
web asnwer: SUPPORTS
wiki asnwer: REFUTES

web provenance:
 diners - or restaurant inspectors, as we better know them today - to visit and review restaurants anonymously. In 1926, the guide began to award stars for fine dining establishments, initially marking them only with a single star. Five years later, a hierarchy of zero, one, two, and three stars was introduced, and in 1936, the criteria for the starred rankings were published. During the rest of 20th century, thanks to its serious and unique approach, the MICHELIN Guides became best-sellers without equals: the guide now rates over 30,000 establishments in over 30 territories across three continents, and more than
https://guide.michelin.com/it/en/about-us

wiki provenance:
 Michelin Guide Michelin Guides ( ) are a series of guide books published by the French tire company for more than a century. The term normally refers to the annually published Michelin "Red Guide", the oldest European hotel and restaurant reference guide, which awards up to three "Michelin stars" for excellence to a select few establishments. The acquisition or loss of a star can have dramatic effects on the success of a restaurant. Michelin also publishes a series of general guides to cities, regions, and countries, the
Michelin Guide

==> tables/reader_dev.tex <==
\begin{table*}[t!]
\centering
\resizebox{0.75\linewidth}{!}{    
    \fontsize{8.4}{10.1}\selectfont \setlength{\tabcolsep}{0.5em}
\begin{tabular}{ccccccccc}
 \toprule
 \multicolumn{2}{r}{Fact Check.}  & \multicolumn{2}{c}{Slot Filling} & \multicolumn{4}{c}{Open Domain QA} & \multicolumn{1}{c}{Dial.}  \\
 model  & \textbf{\fever}  & \textbf{\trex} & \textbf{\zsre}  & \textbf{\nq} & \textbf{\hotpot} & \textbf{\trivia} & \textbf{\eli}  & \textbf{\wow}   \\

\midrule
& \multicolumn{3}{c}{Accuracy} & \multicolumn{3}{c}{Exact Match} & \multicolumn{1}{c}{RL} & \multicolumn{1}{c}{F1} \\
\midrule
 
\multicolumn{9}{c}{\textbf{Wikipedia}} \\
\midrule
\fidmulti & 90.48 & 81.90 & 70.73 & 55.55 & 37.41 & 69.92 & 18.12 & 15.92 \\
\fidweb &90.93 & 80.94 & 72.39 & 54.98 & 38.04 & 71.43 & 17.88 & 16.11 \\
\midrule
\multicolumn{9}{c}{\textbf{\sphere}} \\
\midrule
\fidmulti & 87.64 & 49.86 & 23.23 & 46.60 & 27.73 & 68.73 & 18.02 & 15.46 \\
\fidweb & 89.67 & 54.62 & 33.14 & 49.07 & 31.84 & 72.57 & 18.07 & 15.34 \\
\fidbm & 90.71 & 59.66 & 38.61 & 46.28 & 34.12 & 78.43 & 17.13 & 17.82 \\
%\midrule
%\multicolumn{9}{c}{\textbf{Wikipedia + \sphere} (upper bound)} \\
%\midrule
%hybrid & 94.52 & 85.40 & 77.58 & 65.10 & 47.84 & 86.58 & 20.60 & 22.59 \\
\bottomrule
\end{tabular}
}
\caption{Downstream evaluation results on the dev set.}
\label{tab:reader_dev}
\end{table*}

==> tables/retrieval_dev.tex <==
\begin{table*}[t!]
\centering
\resizebox{\columnwidth}{!}{    
    \fontsize{8.4}{10.1}\selectfont \setlength{\tabcolsep}{0.5em}
\begin{tabular}{cccccc}
 \toprule
 model  & \textbf{\trex} & \textbf{\zsre}  & \textbf{\nq} & \textbf{\hotpot} & \textbf{\trivia}  \\

\midrule
\multicolumn{6}{c}{\aic{@1}} \\

\midrule
 
\multicolumn{6}{c}{\textbf{Wikipedia}} \\
\midrule
\fidmulti & 79.22 & 63.50 & 54.18 & 30.62 & 69.79 \\
\fidweb & 84.28 & 75.54 & 58.48 & 35.48 & 73.13 \\
\midrule
\multicolumn{6}{c}{\textbf{\sphere}} \\
\midrule
\fidmulti & 40.08 & 12.03 & 37.72 & 17.62 & 61.73 \\
\fidweb & 57.5 & 28.44 & 53.61 & 30.30 & 78.99 \\
\fidbm & 42.32 & 22.45 & 27.21 & 25.36 & 67.66 \\

\bottomrule
\end{tabular}
}
\caption{Retriever models - \aic{@1} on the dev set.}
\label{tab:retrieval_dev}
\end{table*}

==> tables/retrieval_test.tex <==
\begin{table*}[t!]
\centering
\resizebox{0.75\linewidth}{!}{    
    \fontsize{8.4}{10.1}\selectfont \setlength{\tabcolsep}{0.5em}
\begin{tabular}{ccccccccc}

\toprule
%\multicolumn{2}{r}{Fact Check.}  & \multicolumn{2}{c}{Slot Filling} & \multicolumn{4}{c}{Open Domain QA} & \multicolumn{1}{c}{Dial.}  \\

models & \textbf{\fever}  & \textbf{\trex} & \textbf{\zsre}  & \textbf{\nq} & \textbf{\hotpot} & \textbf{\trivia} & \textbf{\eli}  & \textbf{\wow}   \\

\midrule

\multicolumn{9}{c}{R-precision / {\textbf{Wikipedia}}} \\

\midrule

\multicolumn{9}{c}{\textbf{test}} \\
\midrule
\fidmulti & 74.77 & 71.86 & 83.14 & 58.59 & 45.38 & 59.67 & 14.83 & 41.54 \\
\fidweb & 72.03 & 75.64 & 89.63 & 59.83 & 47.23 & 58.85 & 14.00 & 36.71 \\


\midrule
\multicolumn{9}{c}{\textbf{dev}} \\
\midrule
\fidmulti & 70.78 & 72.28 & 81.26 & 59.74 & 45.30 & 59.94 & 14.53 & 41.19 \\
\fidweb & 73.56 & 74.80 & 89.66 & 60.80 & 47.03 & 58.07 & 13.07 & 37.95 \\


\bottomrule
\end{tabular}
}
\caption{R-precision retrieval evaluation results on the test set as per KILT leaderboard.}
\label{tab:retrieval_test}
\end{table*}

